Generating Upper-Body Motion for Real-Time Characters Making their Way through Dynamic Environments

Real-time character animation in dynamic environments requires the generation of plausible upper-body movements regardless of the nature of the environment, including non-rigid obstacles such as vegetation. We propose a flexible model for upper-body interactions, based on the anticipation of the character's surroundings, and on antagonistic controllers to adapt the amount of muscular stiffness and response time to better deal with obstacles. Our solution relies on a hybrid method for character animation that couples a keyframe sequence with kinematic constraints and lightweight physics. The dynamic response of the character's upper-limbs leverages antagonistic controllers, allowing us to tune tension/relaxation in the upper-body without diverging from the reference keyframe motion. A new sight model, controlled by procedural rules, enables high-level authoring of the way the character generates interactions by adapting its stiffness and reaction time. As results show, our real-time method offers precise and explicit control over the character's behavior and style, while seamlessly adapting to new situations. Our model is therefore well suited for gaming applications.

==> Text/08-Discussion.tex <==
\section{Discussion and Limitations}

% 1.
% About optimizing relaxation for given obstacles - is linear relation enough? Use of RL? - Extension of antagonistic control to the rest of limbs. 

% 2.
% DR: I don’t have clear argument to say why this sphere-like model would be better than a classical rendering in the eye viewspace. And it would be much faster as run on the GPU - we may want to acknowledge that in the limitation.
% Sphere-like model vs classical rendering in the eye viewspace (faster on the GPU)

% 3.
% Non-flat surfaces with hermite interpolation can lead to collisions

% 4. 
% MP: Why "should be" at static equilibrium? This may be our choice to model interactions as series of static equilibrium states; but we can also interact with objects while never being at static equilibrium, such as when a footballer shoots. May be you only mean that the antagonist controller should be at equilibrium?
% DR: If you wanted to model a foot-baller shooting a balloon, then you shouldn’t aim for a controller at equilibrium, but a controller applying an objective torque torque = torque_objective when theta = theta_kin, and with a non zero angular velocity  theta =  theta_objective. This would be more general, but it would change the constraint (actually this would be a "real" extension of the antagonist controller formulation compared to the original article)

\changes{TODO}
